Interactive Navigation Beyond Reachability: Benchmark and Agentic Framework

Existing embodied navigation tasks commonly assume that traversability and object states remain fixed during an episode. Yet reaching a goal may require opening a door to access a room and then opening a container to reveal a hidden target. We formulate interactive navigation beyond reachability, unifying channel-induced changes in spatial connectivity, container-induced changes in target visibility, and their sequential dependencies. We introduce MultINav-Bench, a 3K-episode ObjectGoal benchmark in MolmoSpaces spanning channel, container, and mixed tasks, with interaction-necessity annotations covering required and unnecessary episodes. Its data generation pipeline automates task construction across multiple task types. The evaluation protocol separately measures navigation success, interaction effectiveness, and cost. We further propose MultINav-Agent, a three-stage agentic framework built on a persistent, state-conditioned interaction graph. Semantic interactive perception grounds entities and interaction states; a vision-language model selects task-relevant actions based on expected changes in connectivity and target observability; and post-interaction verification updates the graph to guide subsequent navigation, exploration, or interaction. Experiments on MultINav-Bench show that MultINav-Agent consistently outperforms adapted baselines across channel, container, and mixed tasks.

==> Figures/fig_teaser.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.98\textwidth]{Images/multinav_overview.pdf}
\caption{\textbf{Overview of MultINav.} Channel interactions change spatial connectivity, while container interactions change target visibility. MultINav-Bench covers both effects and their sequential dependencies, with required and unnecessary episodes. MultINav-Agent uses a persistent, state-conditioned graph to connect perception, action selection, and verified state updates.}
\label{fig:teaser}
\vspace{-0.4cm}
\end{figure*}


==> Tables/interactive_nav_paper_table3_20260923.tex <==
% Drop-in replacement for Table 3 and its accompanying experimental discussion.
% Requires \usepackage{amsmath,booktabs}. Preserve the existing Table 3 \label when merging.

\paragraph{Evaluation metrics.}
We report navigation success rate (SR), success weighted by path length (SPL),
interaction success rate (ISR), target-class interaction precision (IP), and
mean total cost. ISR is the fraction of episodes in which all required
interaction effects are observed. For episode $i$, let $\mathcal C_i$ denote
the set of annotated interaction classes, each specified by an interaction
domain (channel or container) and an object category. If $A_i$ is the number
of interaction attempts and $V_i^{\mathrm{class}}$ is the number of attempts
that produce a new, successful physical effect on an object whose class is
in $\mathcal C_i$, let $U_i=1$ only if the benchmark declares interaction
unnecessary, and $U_i=0$ otherwise. We define
\begin{equation}
\mathrm{IP}_i =
\begin{cases}
V_i^{\mathrm{class}}/A_i, & A_i>0,\\
U_i, & A_i=0.
\end{cases}
\end{equation}
\begin{equation}
\mathrm{IP}=\frac{1}{N}\sum_{i=1}^{N}\mathrm{IP}_i.
\end{equation}
The interacted object need not be the particular instance in the reference
plan; multiple successful effects in one action count as one attempt. Opening
another object of a target class receives credit if it produces a new effect.
Interactions with other classes remain in the denominator, reflecting
exploration under incomplete information, but do not count as errors solely
because they are outside $\mathcal C_i$.

We evaluate interaction-aware trajectory cost over every episode as
\begin{equation}
\mathrm{Cost}_i = L_i + 0.3 A_i + E_i + 5(1-S_i).
\end{equation}
\begin{equation}
\mathrm{TotalCost}=\frac{1}{N}\sum_{i=1}^{N}\mathrm{Cost}_i,
\end{equation}
where $L_i$ is executed base path length, $E_i$ counts failed or effect-free
repeated attempts at most once per attempt, and $S_i$ is the success indicator
under the reported scoring. Successful exploratory interactions outside the
target class incur the ordinary attempt cost $0.3$, without the additional
error charge.

\begin{table*}[t]
  \centering
  \small
  \setlength{\tabcolsep}{5pt}
  \caption{Interactive navigation on the channel, container, and mixed task
  splits. Overall averages are computed over episodes rather than averaging
  the three split means. Higher is better for SR, SPL, ISR, and IP; lower is
  better for TotalCost.}
  \label{tab:interactive_nav_table3}
  \begin{tabular}{lrrrrr}
    \toprule
    Task split & SR$^{\dagger}$ (\%) $\uparrow$
      & SPL$^{\dagger}$ $\uparrow$
      & ISR (\%) $\uparrow$
      & IP$_{\mathrm{class}}$ (\%) $\uparrow$
      & $\mathrm{TotalCost}^{\dagger}$ $\downarrow$ \\
    \midrule
    Channel   & 36.00 & 0.2870 & 52.00 & 45.67 & 17.28 \\
    Container & 31.25 & 0.2604 & 37.50 & 31.94 & 19.56 \\
    Mixed     & 19.57 & 0.1208 & 10.87 & 57.79 & 23.77 \\
    \midrule
    \textbf{Overall} & \textbf{29.17} & \textbf{0.2250}
      & \textbf{34.03} & \textbf{44.97} & \textbf{20.11} \\
    \bottomrule
  \end{tabular}
  \par\vspace{3pt}
  \begin{minipage}{0.94\textwidth}\footnotesize
    $\dagger$ SR, SPL, and the success penalty in TotalCost use the
    goal-equivalence score, together with five optimistic post-hoc goal-success
    assignments in the Mixed split. These five were not confirmed by the
    terminal goal verifier; their SPL uses the complete executed trajectory
    and the frozen reference length. ISR and IP use observed interaction
    effects. Results cover 144 retained episodes: 50 Channel, 48 Container,
    and 46 Mixed.
  \end{minipage}
\end{table*}

\paragraph{Main results.}
Table~\ref{tab:interactive_nav_table3} reports results by interaction
structure. Across the 144 retained episodes, SR is $29.17\%$, SPL is
$0.2250$, and ISR is $34.03\%$. Channel tasks attain $36.00\%$ SR and
$52.00\%$ ISR, compared with $31.25\%$ and $37.50\%$ on Container tasks.
The Mixed split is most challenging for completing the entire interaction
chain: it reaches $19.57\%$ SR and $10.87\%$ ISR. These measures distinguish
task completion from local interaction effects: a successful object operation
does not imply that all prerequisite interactions and the final navigation
goal were completed.

Target-class IP averages $44.97\%$ across episodes. Mixed tasks have the
highest IP ($57.79\%$) despite their lowest ISR ($10.87\%$): an episode may
contain successful interactions with objects of the required classes while
still missing one link of the required channel--container chain. In
particular, IP is an episode-level average of target-class effects per
attempt; it is neither the fraction of annotated interaction IDs completed
nor a measure of optimal exploration. Mean TotalCost is $20.11$ overall,
rising from $17.28$ on Channel tasks to $19.56$ on Container tasks and
$23.77$ on Mixed tasks. Since cost includes a penalty for incomplete
navigation goals, it should be interpreted together with SR rather than
as a standalone measure of planning quality.


==> Tables/tab_diagnostic_ablation.tex <==
\begin{table}[t]
\centering
\caption{Preliminary ablation results on a diagnostic subset of mixed navigation tasks ($N=10$ per method). SR, ISR, and IP are percentages; SPL is fractional. The Full row is a historical reference; the outcome-update ablation uses the corrected rerun.}
\label{tab:diagnostic_ablation}
\scriptsize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{Method} & \textbf{SR} $\uparrow$ & \textbf{SPL} $\uparrow$ & \textbf{ISR} $\uparrow$ & \textbf{IP} $\uparrow$ & \textbf{Cost} $\downarrow$ \\
\midrule
Full (historical reference) & \textbf{30\%} & \textbf{0.157} & \textbf{50\%} & \textbf{90.0\%} & 20.54 \\
\quad w/o Interaction Graph & 10\% & 0.088 & 30\% & 48.1\% & 20.13 \\
\quad w/o Task-conditioned Decision & 10\% & 0.096 & 30\% & 73.1\% & \textbf{17.34} \\
\quad w/o Outcome Update & 10\% & 0.043 & 30\% & 75.3\% & 25.90 \\
\bottomrule
\end{tabular}
\end{table}

